Algebraic Pattern Matching in Join Calculus

We propose an extension of the join calculus with pattern matching on algebraic data types. Our initial motivation is twofold: to provide an intuitive semantics of the interaction between concurrency and pattern matching; to define a practical compilation scheme from extended join definitions into ordinary ones plus ML pattern matching. To assess the correctness of our compilation scheme, we develop a theory of the applied join calculus, a calculus with value passing and value matching. We implement this calculus as an extension of the current JoCaml system.

==> Makefile <==
#oojoin_typing.dvi: oojoin_typing.tex oojoin_typing.bbl
#	./fixlatex oojoin_typing.tex

#oojoin_typing.html: oojoin_typing.tex oojoin_typing.bbl
#	hevea ....... oojoin_typing.tex

#oojoin_typing.bbl: oojoin.bib
#	latex oojoin_typing.tex
#	bibtex oojoin_typing    # -min-crossrefs=0 
#	/bin/rm -f oojoin_typing.dvi
#	$(MAKE) $(MFLAGS)  oojoin_typing.dvi
FILE=pt-join
FIGS=dag.fig bisi.fig bisi2.fig ejocaml_flow.fig redbisiuptoid.fig wbcuptoequiv.fig wbcuptoid.fig wbcuptoequiv-alt.fig wbbisi-alt.fig
PACK_NAME=$(FILE).tar.gz

LATEX=latex < /dev/null
PDFLATEX=pdflatex < /dev/null

all: bib pdf
dvi: $(FILE).dvi
ps: $(FILE).ps
pdf: $(FILE).pdf

FIGS_EPS=$(FIGS:.fig=.eps)
FIGS_PSTEX_T=$(FIGS:.fig=.fex)

$(FILE).dvi: $(FIGS_EPS) $(FIGS_PSTEX_T)
$(FILE).ps: $(FIGS_EPS)

bib: $(FILE).dvi
	bibtex $(FILE)
	/bin/rm -f $(FILE).dvi
	$(MAKE) $(FILE).dvi

clean::
	rm -f *.aux *.log *~ *.dvi *.ps *.bbl *.blg *.aux *.pdf $(FIGS_EPS) $(FIGS_PSTEX_T) $(PACK_NAME) $(FILE).out

FILES=Makefile pt-join.tex ptjoin.bib\
 lmcs.cls listings.sty lstjoin.sty lstmisc.sty lstpatch.sty mathpartir.sty\
 url.sty hyperref.cfg pd1enc.def hyperref.sty hdvips.def pdfmark.def\
 listings.cfg  lstlocal.cfg\
 $(FIGS)
pack: $(FILES)
	mkdir -p $(FILE)
	cp $(FILES) $(FILE)
	cd $(FILE) && make bib pdf && /bin/rm -f ptjoin.bib pt-join.out
	tar -zcf $(PACK_NAME) $(FILE)
#	/bin/rm -rf $(FILE)

.SUFFIXES: .tex .dvi .pstex_t .eps .ps .fig .pdf .fex

.tex.dvi:
	$(LATEX) $*.tex
	grep Rerun $*.log && $(LATEX) $*.tex || echo OK
	grep Rerun $*.log && $(LATEX) $*.tex || echo OK

.ps.pdf:
	ps2pdf $< $@

.dvi.ps:
	dvips -V -o $@ $<

.fig.eps:
	fig2dev -L pstex $*.fig $*.eps

.fig.fex:
	fig2dev -L pstex_t -p $*.eps $*.fig $*.fex


